Mining and Analyzing the Italian Parliament: Party Structure and Evolution

The roll calls of the Italian Parliament in the XVI legislature are studied by employing multidimensional scaling, hierarchical clustering, and network analysis. In order to detect changes in voting behavior, the roll calls have been divided in seven periods of six months each. All the methods employed pointed out an increasing fragmentation of the political parties endorsing the previous government that culminated in its downfall. By using the concept of modularity at different resolution levels, we identify the community structure of Parliament and its evolution in each of the considered time periods. The analysis performed revealed as a valuable tool in detecting trends and drifts of Parliamentarians. It showed its effectiveness at identifying political parties and at providing insights on the temporal evolution of groups and their cohesiveness, without having at disposal any knowledge about political membership of Representatives.

==> refs.tex <==
\begin{thebibliography}{10}

\bibitem{Brazill2002}
Timothy~J. Brazill and Bernard Grofman.
\newblock Factor analysis versus multi-dimensional scaling: binary choice
  roll-call voting and the us supreme court.
\newblock {\em Social Networks}, 24(3):201 -- 229, 2002.

\bibitem{Fortunato2007a}
S.~Fortunato and M.~Barth\'elemy.
\newblock Resolution limit in community detection.
\newblock {\em Proc. National Academy of Science, USA}, 104(36), 2007.

\bibitem{Granel2012}
C.~Granell, S.~G\'omez, and A.~Arenas.
\newblock Unsupervised clustering analisys : A multiscale complex network
  approach.
\newblock {\em Journal of Bifurcation and Chaos, in press}, 2012.

\bibitem{Hix2005}
Simon Hix, Abdul Noury, and G\'erard Roland.
\newblock Power to the parties: Cohesion and competition in the {E}uropean
  {P}arliament.
\newblock {\em British Journal of Political Science}, 35(2), 2005.

\bibitem{jain-88}
A.K. Jain and R.~Cg Dubes.
\newblock {\em Algorithms for Clustering Data}.
\newblock Prentice Hall, 1988.

\bibitem{Jak2004}
Aleks Jakulin and Wray Buntine.
\newblock Analyzing the {US} {S}enate in 2003: Similarities, networks, clusters
  and blocs.
\newblock {\em http://eprints.fri.uni-lj.si/archive/00000146/}, 2004.

\bibitem{kauf1990}
L.~Kauffman and P.~J. Rousseeuw.
\newblock {\em Finding Groups in Data}.
\newblock Wiley, New York, 1990.

\bibitem{Macon2012}
K.~T. Macon, P.~J. Mucha, and M.~A. Porter.
\newblock Community structure in {U}nited {N}ations {G}eneral {A}ssembly.
\newblock {\em Physica A: Statistical Mechanics and its Applications},
  391(1-2):343--361, January 2012.

\bibitem{NewmanGirvan2004}
M.~E.~J. Newman and M.~Girvan.
\newblock Finding and evaluating community structure in networks.
\newblock {\em Physical Review}, E69:026113, 2004.

\bibitem{Pajala04}
Antti Pajala, Aleks Jakulin, and Wray Buntine.
\newblock Parliamentary group and individual voting behavior in {F}innish
  {P}arliament in year 2003 : A group cohesion and voting similarity analysis.
\newblock {\em
  http://citeseerx.ist.psu.edu/viewdoc/summary?doi=10.1.1.103.2295}, 2004.

\bibitem{pizzuti2012}
C.~Pizzuti.
\newblock Boosting the detection of modular community structure with genetic
  algorithms and local search.
\newblock In {\em Proc. of the 27th Symposium on Applied Computing (SAC 2012)},
  pages 226--231, 2012.

\bibitem{Porter2007}
M.~A. Porter, P.J. Mucha, M.~E.~J. Newman, and A.~J. Friend.
\newblock Community structure in the {U}nited {S}tates {H}ouse of
  {R}epresentatives.
\newblock {\em Physica A: Statistical Mechanics and its Applications},
  386(1):414--438, December 2007.

\bibitem{Rajiski1961}
C.~Rajiski.
\newblock Community structure in {C}ongressional cosponsorship networks.
\newblock {\em Information and Control}, 4:373--377, 1991.

\bibitem{Shannon1948}
C.~Shannon.
\newblock A mathematical theory of computation.
\newblock {\em The Bell System Technical Journal}, 27:623--656, 1948.

\bibitem{Strang2005}
G.~Strang.
\newblock {\em Linear Algebra and its Applications}.
\newblock IV edition, Thomson Brooks/Cole, 2005.

\bibitem{tan06}
P.~Tan, M.~Steinbach, and V.~Kumar.
\newblock {\em Introduction to Data Mining}.
\newblock Pearson International Edition, 2006.

\bibitem{Wass2009}
S.~Wasserman and K.~Faust.
\newblock {\em Social Network Analysis - Methods and Applications}.
\newblock Cambridge University Press, 2009.

\bibitem{watt98}
D.J. Watts and S.~H. Strongatz.
\newblock Collective dynamics of 'small-world' networks.
\newblock {\em Nature}, 6684(393):440--442, 1998.

\bibitem{WPFMP09}
A.~S. Waugh, L.~Pei, J.~H. Fowler, P.~J. Mucha, and M.~A. Porter.
\newblock Party polarization in {C}ongress: A network science approach.
\newblock {\em http://arxiv.org/abs/0907.3509}, 2009.

\bibitem{Zhang2008}
Y.~Zhang, A.J. Friend, A.~L. Traud, M.~A. Porter, J.~H. Fowler, and P.~J.
  Mucha.
\newblock Community structure in {C}ongressional cosponsorship networks.
\newblock {\em Physica A: Statistical Mechanics and its Applications},
  387(7):1705--1712, 2008.

\end{thebibliography}
